Lightweight Delivery Detection on Doorbell Cameras

Despite recent advances in video-based action recognition and robust spatio-temporal modeling, most of the proposed approaches rely on the abundance of computational resources to afford running huge and computation-intensive convolutional or transformer-based neural networks to obtain satisfactory results. This limits the deployment of such models on edge devices with limited power and computing resources. In this work we investigate an important smart home application, video based delivery detection, and present a simple and lightweight pipeline for this task that can run on resource-constrained doorbell cameras. Our method relies on motion cues to generate a set of coarse activity proposals followed by their classification with a mobile-friendly 3DCNN network. To train we design a novel semi-supervised attention module that helps the network to learn robust spatio-temporal features and adopt an evidence-based optimization objective that allows for quantifying the uncertainty of predictions made by the network. Experimental results on our curated delivery dataset shows the significant effectiveness of our pipeline and highlights the benefits of our training phase novelties to achieve free and considerable inference-time performance gains.

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Computer Vision has become potent thanks to advances in Deep Learning to an extent that long standing problems like object detection, semantic segmentation, face and human action recognition can now be solved with high accuracy. Despite this, we have to highlight that this often comes at the price of significant computational burden which is typically accelerated by the use of Graphical Processing Units (GPU), Tensor Processing Units (TPU), or Neural Processing Units (NPU). Therefore, the degree to which computer vision tasks can be solved on edge devices with limited resources and computational power is constrained. Among these tasks is \textbf{Delivery Detection} which is concerned with recognizing delivery of merchandises (package, food, groceries, mail, etc. ) at front doors to provide timely notifications for customers. Note that delivery detection task is different from package detection in that it identifies the instances of delivering items rather than the mere detection of packages which is currently practiced in smart home solutions. Delivery detection has numerous advantages including prevention of food perishing and porch piracy to name a few. According to the package theft annual report\footnote{{\scriptsize\url{https://security.org/package-theft/annual-report/}}}, in a twelve month period from 2021 to 2022, there has been more than 49 million package theft incidents in the United States alone with the estimated value of $\$2.4$B. The prevalence of smart devices including smart doorbell and security cameras through out houses facilitates the development and adoption of automated delivery detection systems which can significantly reduce losses. Fig. \ref{fig:sample_deliveries} shows captured deliveries by doorbell cameras.  
\begin{figure}[t!]
    \centering
    \subfloat{\includegraphics[width=.11\textwidth, height=.11\textwidth]{Amazon.png}}~
    \subfloat{\includegraphics[width=0.11\textwidth, height=.11\textwidth]{usps.png}}~
    \subfloat{\includegraphics[width=0.11\textwidth, height=.11\textwidth]{fedex.png}}~
    \subfloat{\includegraphics[width=0.11\textwidth, height=.11\textwidth]{ups.png}}
    \caption{Sample delivery events captured by doorbell cameras.}
    \label{fig:sample_deliveries}
\end{figure}
Despite potential applications, delivery detection is a challenging task. Type, shape and size of packages can be quite diverse. Cardboard boxes in various size, mail, grocery bags, and food are among the items that are frequently being delivered. Additionally, there are various courier services including United States Postal Services (USPS), United Parcel Services (UPS), DHL and Amazon, as well growing number of smaller companies like DoorDash and Uber Eats especially after the COVID-19 pandemic. 
This translates to delivery personnel having diverse outfits and appearances as evidenced by Fig. \ref{fig:sample_deliveries}. Finally the temporal extent of delivery events have high variance. Smaller items are delivered in a matter of seconds while delivering heavier objects can take much longer in the order of minutes. This also depends on submitting the proof of delivery in the form of a picture. Existing solutions such as Ring, Nest Hello, Arlo, AWS Rekognition, and Vivint mainly require cloud processing which results in higher bandwidth utilization, computation, and increased subscription fees. In addition, transferring data creates privacy concerns as opposed to local processing. Moreover, these methods primarily focus on detecting packages/boxes and not the instances of deliveries. In addition, package detection may fail as small or occluded packages are harder to be detected. Therefore, we set out to propose a solution to detect delivery instances that can be implemented on edge devices. We present a lightweight system that relies on motion detection to generate event proposals followed by their classification with a mobile-friendly 3DCNN \cite{ji20123d} network. Through the novel incorporation of an attention mechanism and benefiting from the the theory of evidence and subjective logic, we significantly improve the base performance of this system without imposing additional processing. In summary, this paper makes the following contributions:
\begin{itemize}
    \item We introduce a lightweight delivery detection system running on doorbell cameras with ARM Cortex-A family of processors. In contrast to the widely used package detection in the industry, our system is to detect the delivery events from videos.    
    \item We propose a semi-supervised attention module in 3DCNNs to extract robust spatio-temporal features.
    \item We propose to adopt evidential learning objective to quantify the uncertainty of predictions and enforce a minimum certainty score to ensure quality predictions.
\end{itemize}
